Efficient Automated Deep Learning for Time Series Forecasting

Recent years have witnessed tremendously improved efficiency of Automated Machine Learning (AutoML), especially Automated Deep Learning (AutoDL) systems, but recent work focuses on tabular, image, or NLP tasks. So far, little attention has been paid to general AutoDL frameworks for time series forecasting, despite the enormous success in applying different novel architectures to such tasks. In this paper, we propose an efficient approach for the joint optimization of neural architecture and hyperparameters of the entire data processing pipeline for time series forecasting. In contrast to common NAS search spaces, we designed a novel neural architecture search space covering various state-of-the-art architectures, allowing for an efficient macro-search over different DL approaches. To efficiently search in such a large configuration space, we use Bayesian optimization with multi-fidelity optimization. We empirically study several different budget types enabling efficient multi-fidelity optimization on different forecasting datasets. Furthermore, we compared our resulting system, dubbed \system, against several established baselines and show that it significantly outperforms all of them across several datasets.

==> nomclat.tex <==
% Everything supposed to be used in equation mode?
% use in preamble: \input{macros_DAC.tex}

% Necessary packages for definitions
\usepackage{amsmath}
\usepackage{mathtools}  % for :=
\usepackage{amsfonts} 

\newcommand{\code}[1]{\small{\texttt{#1}}} 

%beginmacros

%--------- General Math Notation
\DeclareMathOperator*{\E}{\mathbb{E}}           % Expectation as a math operator
\DeclareMathOperator*{\expectation}{\mathbb{E}} % Expectation as a math operator
\renewcommand{\vec}[1]{\mathbf{#1}}             % Bold emphasis for vectors
\DeclareMathOperator*{\argmin}{arg\,min}        % Argmin
\DeclareMathOperator*{\argmax}{arg\,max}        % Argmax
\newcommand{\natnums}{{\mathbb{N}}}              % Notation for set of natural numbers
\newcommand{\realnums}{{\mathbb R}}             % Notation for set of real numbers
\newcommand{\extset}[2]{\{#1 \; | \; #2\}}      % Set of a given b. Renders {{a | b}}.    
\newcommand{\ddfrac}[2]{\frac{\displaystyle #1}{\displaystyle #2}}    % Double Display Fraction, forces large displays for everything in numerator and denominator

\newcommand{\diff}{\mathop{}\!\mathrm{d}}       % ???????
\newcommand{\transpose}[0]{{\textrm{\tiny{\sf{T}}}}} % Transpose T. Usage: $A^\transpose$
\newcommand{\norm}{{\mathcal{N}}}               % Normal distribution
\newcommand{\normaldist}{{\mathcal{N}}}         % Normal distribution
\newcommand{\iter}[2][\bocount]{{#2}^{(#1)}}    % Iteration specific instance of variable/function/anything

%-- Stochastic
\newcommand{\pdf}{\phi}                         % Standard Normal PDF
\newcommand{\cdf}{\Phi}                         % Standard Normal CDF
\newcommand{\mean}{\mu}                         % Mean
\newcommand{\stddev}{\sigma}                    % Standard Deviation
\newcommand{\variance}{\sigma^2}                % Variance
\newcommand{\noise}{\nu}                        % Noise
\newcommand{\given}[1][]{\:#1\vert\:}           % Conditional Probability "Given That" Relation, source: https://tex.stackexchange.com/a/141685/205886
\newcommand{\prob}[0]{p}                        % Probability p
\newcommand{\Prob}[0]{P}                        % Probability distribution P


%------- Notation for Configuration(s)

\newcommand{\confspace}[0]{\pmb{\Lambda}}       % Configuration space of parameters
\newcommand{\conf}[0]{\pmb{\lambda}}            % Configuration of parameters
%\newcommand{\bx}[0]{\conf}                     % Configuration of parameters
\newcommand{\hyperparam}{\lambda}               % Single hyperparameter of configuration
\newcommand{\hyperparami}[1][i]{{\hyperparam}_{#1}}   % Single hyperparameter within a hyperparameter configuration
\newcommand{\confinc}[0]{\pmb{\hat{\lambda}}}   % Incumbent configuration
%\newcommand{\confI}[1]{{\conf}^{(#1)}}      % Configuration corresponding to a given iteration -- better use \iter!
\newcommand{\confdef}[0]{{\conf}_{\text{def}}}  % Default configuration
\newcommand{\incumbent}[1][\bocount]{\iter[#1]{\confinc}}   % Incumbent configuration
\newcommand{\confincfin}{\incumbent[\bobudget]} % Final incumbent configuration (at end of run)
\newcommand{\confopt}[0]{{\conf}^*}             % Optimal configuration


%------- Notation for Cost, Risk, Loss, Performance Metric or Objective Functions

\newcommand{\loss}[0]{\mathcal{L}}              % Loss
\newcommand{\risk}{\mathcal{R}}                 % Risk
\newcommand{\riskemp}{\mathcal{R}_{\text{emp}}} % Empirical risk
\newcommand{\cost}[0]{c}                        % Cost
\newcommand{\costi}[1]{c^{(#1)}}                % Cost of instance/identifier
\newcommand{\objF}{F}                           % Family of objective functions
\newcommand{\func}[0]{f}                        % Function
\newcommand{\perfdomain}[0]{\mathbb{R}}         % Performance domain


%------- Notation for Algorithms
\newcommand{\algo}[0]{A}                        % One algorithm
\newcommand{\algos}[0]{\mathbf{A}}              % Set of algorithms    


\newcommand{\feat}[0]{\x_{\text{meta}}}                 % Meta features
\newcommand{\feats}[0]{\mathcal{X}_{\text{meta}}}       % Set of meta features


%------- Notation for Machine Learning
\newcommand{\dset}[0]{\mathcal{D}}                          % Dataset (instance)
\newcommand{\dsetmeta}[0]{\dset_{\text{meta}}}              % Dataset: meta
\newcommand{\dsettrain}[0]{\dset_{\text{train}}}            % Dataset: train
\newcommand{\dsetval}[0]{\dset_{\text{val}}}                % Dataset: val
\newcommand{\dsettest}[0]{\dset_{\text{test}}}              % Dataset: test
\newcommand{\x}[0]{\mathbf{x}}                              % Input vector x
\newcommand{\y}[0]{y}                                       % Output y
\newcommand{\xI}[1]{\mathbf{x}^{(#1)}}                      % i-th component of input
\newcommand{\yI}[1]{y^{(#1)}}                               % i-th component of output
\newcommand{\fx}{f(\mathbf{x})}                             % f(x), continuous prediction function
\newcommand{\Hspace}{\mathcal{H}}                           % hypothesis space where f is from
\newcommand{\fh}{\hat{f}}                                   % f hat, estimated prediction function


%------- Notation for Deep Learning
\newcommand{\weights}[0]{\theta}                            % Weights of neural network
\newcommand{\metaweights}[0]{\phi}                          % Weights of a meta-network


%------- Notation for AutoML
\newcommand{\portfolio}[0]{\mathbf{P}}                      % Portfolio
\newcommand{\schedule}[0]{\mathcal{S}}                      % Schedule
\newcommand{\hist}[0]{\dset_{\text{hist}}}                  % History


%------- Notation for Bayesian Optimization
%-- Components
\newcommand{\GP}{\mathcal{G}}                   % Gaussian Process
\newcommand{\kernel}{\kappa}                    % Kernel
\newcommand{\acq}{u}                            % Acquisition Function
\newcommand{\constraintg}{g}                    % Constraint function
\newcommand{\surro}[0]{\hat{\cost}}             % Surrogate model

%-- Loop
\newcommand{\bocount}{t}                        % BO loop counter
\newcommand{\bobudget}{T}                       % BO loop counter max, the counter runs from 1 to this value
\newcommand{\obs}[1][\conf]{\cost({#1})}        % BO loop observation
\newcommand{\obsspace}{\mathcal{Y}}             % BO loop observation space
\newcommand{\bonextobs}{\obs[\iter{\conf}]}     % BO loop next observation
\newcommand{\bonextsample}{\iter{\conf}}        % BO loop next selected sample

%-- Dataset
\newcommand{\dsetHPOdef}{{\langle \bonextsample,\,\bonextobs \rangle}_{\bocount=1}^{\bobudget}}     % Observed cost for selected configurations during BO run


%------- Notation for Reinforcement Learning
%-- Markov Decision Process with Components
\newcommand{\MDP}[0]{\mathcal{M}}                       % MDP (Markov Decision Process)
\newcommand{\statespace}[0]{\mathcal{S}}                % State space
\newcommand{\state}[0]{s}                               % State
\newcommand{\statet}[1][t]{\state_{#1}}                 % State at time t
\newcommand{\actionspace}[0]{\mathcal{A}}               % Action space
\newcommand{\actionrl}[0]{a}                            % Action
\newcommand{\transdomain}[0]{\mathcal{T}}               % Transition domain (probability distribution of algorithm state transitions)
\newcommand{\trans}[0]{t}                               % Transition
\newcommand{\rewards}[0]{\mathcal{R}}                   % Reward function
\newcommand{\reward}[0]{r}                              % Reward

\newcommand{\policies}[0]{\mathbf{\Pi}}                 % Policies
\newcommand{\policy}[0]{\pi}                            % Policy
\newcommand{\policyopt}[0]{{\policy}^*}                 % Optimal policy

\newcommand{\discount}[0]{\gamma}                       % Discount rate
\newcommand{\valueS}[0]{\mathcal{V}}                    % State value function
\newcommand{\valueSip}[1][\inst]{\valueS^{\policy}_{#1}} % State value function under policy pi and instance i
\newcommand{\Qfunc}[0]{\mathcal{Q}}                     % State action value function (Q)
\newcommand{\Qfuncip}[1][\inst]{\Qfunc^{\policy}_{#1}}  % State action value function (Q) under policy pi and instance i

\newcommand{\egreedy}[0]{$\epsilon$-greedy}             % $\egreedy$ 

\newcommand{\trajectory}{\tau}                          % Trajectory
\newcommand{\episode}[0]{\mathcal{E}}                  % Episode
\newcommand{\expreturn}[0]{G}                           % Expected return
\newcommand{\cutoff}[0]{\kappa}                         % Cutoff kappa


%-- Dynamic Algorithm Configuration (DAC)
\newcommand{\inst}[0]{i}                    % One instance
\newcommand{\insts}[0]{\mathcal{I}}         % Set of instances
\newcommand{\insti}[1]{i^{(#1)}}            % Numbered instance. Usage: $\insti{3}$ for 3rd instance.

\newcommand{\cMDP}[0]{\MDP_\insts}                      % cMDP (contextual MDP)
\newcommand{\cMDPdef}[0]{\cMDP \coloneqq \{\MDPi\}_{\inst \sim \insts}} % cMDP: Definition as set of MDPs per instance
\newcommand{\MDPi}[0]{\MDP_\inst}                       % MDP of one instance
\newcommand{\MDPidef}[0]{\MDPi \coloneqq (\statespace, \actionspace, \transdomaini, \rewardsi)}  % MDP: Definition as tuple for one instance

\newcommand{\transdomaini}[0]{\transdomain_\inst}       % Transitions (instance-specific)
\newcommand{\rewardsi}[0]{\rewards_\inst}               % Rewards (instance-specific)    
\newcommand{\curric}[0]{\mathbf{d}}                     % Curriculum
\newcommand{\contexti}[1][i]{c_{#1}}                    % Context of instance i

\newcommand{\configspaceDAC}[0]{\Theta}                 % Configuration space
\newcommand{\configDAC}[0]{\theta}                      % Configuration
\newcommand{\hyperparamset}{H}                          % Hyperparameter set
\newcommand{\hyperparamname}[0]{h}                      % Name of hyper-/configuration parameter

%endmacros


% Regret
% Return

==> nomclat_loc.tex <==
% Everything supposed to be used in equation mode?
% use in preamble: \input{macros_DAC.tex}

% Necessary packages for definitions
\usepackage{amsmath}
\usepackage{mathtools}  % for :=
\usepackage{amsfonts} 

\newcommand{\code}[1]{\small{\texttt{#1}}} 

%beginmacros

%--------- General Math Notation
\DeclareMathOperator*{\E}{\mathbb{E}}           % Expectation as a math operator
\DeclareMathOperator*{\expectation}{\mathbb{E}} % Expectation as a math operator
\renewcommand{\vec}[1]{\mathbf{#1}}             % Bold emphasis for vectors
\DeclareMathOperator*{\argmin}{arg\,min}        % Argmin
\DeclareMathOperator*{\argmax}{arg\,max}        % Argmax
\newcommand{\natnums}{{\mathbb{N}}}              % Notation for set of natural numbers
\newcommand{\realnums}{{\mathbb R}}             % Notation for set of real numbers
\newcommand{\extset}[2]{\{#1 \; | \; #2\}}      % Set of a given b. Renders {{a | b}}.    
\newcommand{\ddfrac}[2]{\frac{\displaystyle #1}{\displaystyle #2}}    % Double Display Fraction, forces large displays for everything in numerator and denominator

\newcommand{\diff}{\mathop{}\!\mathrm{d}}       % ???????
\newcommand{\transpose}[0]{{\textrm{\tiny{\sf{T}}}}} % Transpose T. Usage: $A^\transpose$
\newcommand{\norm}{{\mathcal{N}}}               % Normal distribution
\newcommand{\normaldist}{{\mathcal{N}}}         % Normal distribution
\newcommand{\iter}[2][\bocount]{{#2}^{(#1)}}    % Iteration specific instance of variable/function/anything

%-- Stochastic
\newcommand{\pdf}{\phi}                         % Standard Normal PDF
\newcommand{\cdf}{\Phi}                         % Standard Normal CDF
\newcommand{\mean}{\mu}                         % Mean
\newcommand{\stddev}{\sigma}                    % Standard Deviation
\newcommand{\variance}{\sigma^2}                % Variance
\newcommand{\noise}{\nu}                        % Noise
\newcommand{\given}[1][]{\:#1\vert\:}           % Conditional Probability "Given That" Relation, source: https://tex.stackexchange.com/a/141685/205886
\newcommand{\prob}[0]{p}                        % Probability p
\newcommand{\Prob}[0]{P}                        % Probability distribution P


%------- Notation for Configuration(s)

\newcommand{\confspace}[0]{\pmb{\Lambda}}       % Configuration space of parameters
\newcommand{\conf}[0]{\pmb{\lambda}}            % Configuration of parameters
%\newcommand{\bx}[0]{\conf}                     % Configuration of parameters
\newcommand{\hyperparam}{\lambda}               % Single hyperparameter of configuration
\newcommand{\hyperparami}[1][i]{{\hyperparam}_{#1}}   % Single hyperparameter within a hyperparameter configuration
\newcommand{\confinc}[0]{\pmb{\hat{\lambda}}}   % Incumbent configuration
%\newcommand{\confI}[1]{{\conf}^{(#1)}}      % Configuration corresponding to a given iteration -- better use \iter!
\newcommand{\confdef}[0]{{\conf}_{\text{def}}}  % Default configuration
\newcommand{\incumbent}[1][\bocount]{\iter[#1]{\confinc}}   % Incumbent configuration
\newcommand{\confincfin}{\incumbent[\bobudget]} % Final incumbent configuration (at end of run)
\newcommand{\confopt}[0]{{\conf}^*}             % Optimal configuration


%------- Notation for Cost, Risk, Loss, Performance Metric or Objective Functions

\newcommand{\loss}[0]{\mathcal{L}}              % Loss
\newcommand{\risk}{\mathcal{R}}                 % Risk
\newcommand{\riskemp}{\mathcal{R}_{\text{emp}}} % Empirical risk
\newcommand{\cost}[0]{c}                        % Cost
\newcommand{\costi}[1]{c^{(#1)}}                % Cost of instance/identifier
\newcommand{\objF}{F}                           % Family of objective functions
\newcommand{\func}[0]{f}                        % Function
\newcommand{\perfdomain}[0]{\mathbb{R}}         % Performance domain


%------- Notation for Algorithms
\newcommand{\algo}[0]{A}                        % One algorithm
\newcommand{\algos}[0]{\mathbf{A}}              % Set of algorithms    


\newcommand{\feat}[0]{\x_{\text{meta}}}                 % Meta features
\newcommand{\feats}[0]{\mathcal{X}_{\text{meta}}}       % Set of meta features


%------- Notation for Machine Learning
\newcommand{\dset}[0]{\mathcal{D}}                          % Dataset (instance)
\newcommand{\dsetmeta}[0]{\dset_{\text{meta}}}              % Dataset: meta
\newcommand{\dsettrain}[0]{\dset_{\text{train}}}            % Dataset: train
\newcommand{\dsetval}[0]{\dset_{\text{val}}}                % Dataset: val
\newcommand{\dsettest}[0]{\dset_{\text{test}}}              % Dataset: test
\newcommand{\x}[0]{\mathbf{x}}                              % Input vector x
\newcommand{\y}[0]{y}                                       % Output y
\newcommand{\xI}[1]{\mathbf{x}^{(#1)}}                      % i-th component of input
\newcommand{\yI}[1]{y^{(#1)}}                               % i-th component of output
\newcommand{\fx}{f(\mathbf{x})}                             % f(x), continuous prediction function
\newcommand{\Hspace}{\mathcal{H}}                           % hypothesis space where f is from
\newcommand{\fh}{\hat{f}}                                   % f hat, estimated prediction function


%------- Notation for Deep Learning
\newcommand{\weights}[0]{\boldsymbol{\theta}}                            % Weights of neural network
\newcommand{\metaweights}[0]{\phi}                          % Weights of a meta-network


%------- Notation for AutoML
\newcommand{\portfolio}[0]{\mathbf{P}}                      % Portfolio
\newcommand{\schedule}[0]{\mathcal{S}}                      % Schedule
\newcommand{\hist}[0]{\dset_{\text{hist}}}                  % History


%------- Notation for Bayesian Optimization
%-- Components
\newcommand{\GP}{\mathcal{G}}                   % Gaussian Process
\newcommand{\kernel}{\kappa}                    % Kernel
\newcommand{\acq}{u}                            % Acquisition Function
\newcommand{\constraintg}{g}                    % Constraint function
\newcommand{\surro}[0]{\hat{\cost}}             % Surrogate model

%-- Loop
\newcommand{\bocount}{t}                        % BO loop counter
\newcommand{\bobudget}{T}                       % BO loop counter max, the counter runs from 1 to this value
\newcommand{\obs}[1][\conf]{\cost({#1})}        % BO loop observation
\newcommand{\obsspace}{\mathcal{Y}}             % BO loop observation space
\newcommand{\bonextobs}{\obs[\iter{\conf}]}     % BO loop next observation
\newcommand{\bonextsample}{\iter{\conf}}        % BO loop next selected sample

%-- Dataset
\newcommand{\dsetHPOdef}{{\langle \bonextsample,\,\bonextobs \rangle}_{\bocount=1}^{\bobudget}}     % Observed cost for selected configurations during BO run


%------- Notation for Reinforcement Learning
%-- Markov Decision Process with Components
\newcommand{\MDP}[0]{\mathcal{M}}                       % MDP (Markov Decision Process)
\newcommand{\statespace}[0]{\mathcal{S}}                % State space
\newcommand{\state}[0]{s}                               % State
\newcommand{\statet}[1][t]{\state_{#1}}                 % State at time t
\newcommand{\actionspace}[0]{\mathcal{A}}               % Action space
\newcommand{\actionrl}[0]{a}                            % Action
\newcommand{\transdomain}[0]{\mathcal{T}}               % Transition domain (probability distribution of algorithm state transitions)
\newcommand{\trans}[0]{t}                               % Transition
\newcommand{\rewards}[0]{\mathcal{R}}                   % Reward function
\newcommand{\reward}[0]{r}                              % Reward

\newcommand{\policies}[0]{\mathbf{\Pi}}                 % Policies
\newcommand{\policy}[0]{\pi}                            % Policy
\newcommand{\policyopt}[0]{{\policy}^*}                 % Optimal policy

\newcommand{\discount}[0]{\gamma}                       % Discount rate
\newcommand{\valueS}[0]{\mathcal{V}}                    % State value function
\newcommand{\valueSip}[1][\inst]{\valueS^{\policy}_{#1}} % State value function under policy pi and instance i
\newcommand{\Qfunc}[0]{\mathcal{Q}}                     % State action value function (Q)
\newcommand{\Qfuncip}[1][\inst]{\Qfunc^{\policy}_{#1}}  % State action value function (Q) under policy pi and instance i

\newcommand{\egreedy}[0]{$\epsilon$-greedy}             % $\egreedy$ 

\newcommand{\trajectory}{\tau}                          % Trajectory
\newcommand{\episode}[0]{\mathcal{E}}                  % Episode
\newcommand{\expreturn}[0]{G}                           % Expected return
\newcommand{\cutoff}[0]{\kappa}                         % Cutoff kappa


%-- Dynamic Algorithm Configuration (DAC)
% \newcommand{\inst}[0]{i}                    % One instance
\newcommand{\insts}[0]{\mathcal{I}}         % Set of instances
\newcommand{\insti}[1]{i^{(#1)}}            % Numbered instance. Usage: $\insti{3}$ for 3rd instance.

\newcommand{\cMDP}[0]{\MDP_\insts}                      % cMDP (contextual MDP)
\newcommand{\cMDPdef}[0]{\cMDP \coloneqq \{\MDPi\}_{\inst \sim \insts}} % cMDP: Definition as set of MDPs per instance
\newcommand{\MDPi}[0]{\MDP_\inst}                       % MDP of one instance
\newcommand{\MDPidef}[0]{\MDPi \coloneqq (\statespace, \actionspace, \transdomaini, \rewardsi)}  % MDP: Definition as tuple for one instance

\newcommand{\transdomaini}[0]{\transdomain_\inst}       % Transitions (instance-specific)
\newcommand{\rewardsi}[0]{\rewards_\inst}               % Rewards (instance-specific)    
\newcommand{\curric}[0]{\mathbf{d}}                     % Curriculum
\newcommand{\contexti}[1][i]{c_{#1}}                    % Context of instance i

\newcommand{\configspaceDAC}[0]{\Theta}                 % Configuration space
\newcommand{\configDAC}[0]{\theta}                      % Configuration
\newcommand{\hyperparamset}{H}                          % Hyperparameter set
\newcommand{\hyperparamname}[0]{h}                      % Name of hyper-/configuration parameter

%endmacros


% Regret
% Return
